A basic macroeconomic agent-based model for analyzing monetary regime shifts

In macroeconomics, an emerging discussion of alternative monetary systems addresses the dimensions of systemic risk in advanced financial systems. Monetary regime changes with the aim of achieving a more sustainable financial system have already been discussed in several European parliaments and were the subject of a referendum in Switzerland. However, their effectiveness and efficacy concerning macro-financial stability are not well-known. This paper introduces a macroeconomic agent-based model (MABM) in a novel simulation environment to simulate the current monetary system, which may serve as a basis to implement and analyze monetary regime shifts. In this context, the monetary system affects the lending potential of banks and might impact the dynamics of financial crises. MABMs are predestined to replicate emergent financial crisis dynamics, analyze institutional changes within a financial system, and thus measure macro-financial stability. The used simulation environment makes the model more accessible and facilitates exploring the impact of different hypotheses and mechanisms in a less complex way. The model replicates a wide range of stylized economic facts, including simplifying assumptions to reduce model complexity.

==> rest.tex <==
Introduction:

and has been subject of diverse studies of regime shifts \cite{Huber.2017,Stellinga.2021,Paniague.2016}. 

Most discussions set the centre of attention to slight adaptations of the existing monetary system via regulation (e.g.,\cite{Claessens.2013, Rubio.2014, Cerutti.2015}. 

%and agent-based model analysis %\cite{Alexandre.2017, vanderHoog.2018, Krug.2018, Popoyan.2019}.
However, a few also discuss alternative monetary regimes, referring to who should control and how to organize money issuance (e.g., current system \cite{DeutscheBundesbank.2017}, centralized system\cite{Huber.2017} and decentralized system\cite{Paniagua.2016}). The suggestion of alternative regimes dates back to the 19th century and is a reincarnation of the debate between banking and currency school with the evolutionary difference that Fiat money replaced the gold standard.


%To allow for successive extensions of the agent-based model, and 
%Therefore we develop an agent-based model to capture the essential dynamics in a transparent and explicit manner, so to allow successive extensions, and testing of %alternative monetary systems ... 
%requirements 
%-- explicit description (seperation of concern) and easy to  discuss 
%-- capturing the dynamics as concurrent processes including stochasticity 


%ML3
\begin{comment}
= Mention complexity features of financial system (OECD \cite{OECD.2016})

financial market and concurrent processes can be found in ML3
= rule based and has high accessibility
= Key features of ML3 and link to section Material and methods... 

new simulation environment and new way of modeling MABM = rule based = leads to new way to define mechanisms (price etc.)

 and related institutional changes within the current financial system of modern economies and the implication of rebound effects with regard to systemic stability. To specify the purpose of the paper the objects under investigation have to be disambiguated.

3) particular challenges in developing such a agent-based model, stochasticity, continuous time, diverse submodels need to be included, some of which might be based on competing hypotheses,  

4) one solution - using a declarative dsl for developing such a model in combination with a provenance approach (to document the theories behind the different sub-models) and how the sub-models are combined. 

B) Materials and methods
@Oliver
1) ML3 

2) Provenance 

C) The model 
starting with Figure 2 ... (to be revised with the helpf of Oliver, based on the provenance pattern by Pia)  

describing all submodels 

D) Simulation experiments 

again starting with Figure 3 (still to be done provenance about the simulation expeirments), again to be done with the help of Oliver and based on the provenance pattern by Pia 

E) Discussion 

1) Related work (what kind of agent-based models exist in economy and how does the model differ?) 

2) Questioning resilience and stability, how does the particular construction of the model, facilitate to answer crucial questions in the context of resilience and stability of money systems 
\end{comment}


To explore the implications of installing such alternative regimes poses serious challenges. 

%The analysis of the monetary system comes along with 
The complexity of the system is also reflected in debates about the nature of money and who should control money issuance or how it should be organized (\cite{Benes and Kumhof)}.\footnote{For further details on the nature of money please see Benes and Kumhof (2012)...ADD further literature.} 
%Lin: is the following what you wanted to say?
%Current analyses of alternative monetary systems sheds new light on the required institutional and regulatory interplay with regard to stability concerns \cite{}.  
%Lin: are these the two we are going to analyze?
There are two contrary monetary systems that both claim to lead to a more stable financial system than the current one when implemented: Sovereign money and Freebanking system \cite{}. A sovereign money system (SMS) is also known as positive money and describes a money system under full money issuance control by the sovereign.
In contrast, a Free banking system (FBS) indicates a pure private money issuance regime
and little or no sovereign interference. 
%Lin: what is the current one? 


%ML3 DESCRIPTION

%TODO include overview of MABM = Dawid and Delli Gatti (2018). To our knowledge we do not know an MABM that is not an discrete-time models.
%Most (TODO: all? and cite) of the aforementioned models are discrete-time models, where time advances in steps, and all agents are updated in some order each step.
%Law \cite{Law2014} stresses two disadvantages of this method:
%First, as in the real world system the model shall represent time does usually not advance in discrete steps, the approach introduces an error in the timing of events.
%Events that should happen between to time steps will instead be moved to the time of the next step.
%Hence, the size of the time-step (e.g., yearly, monthly or daily updates) can also have a significant influence on the model's behavior \cite{Ozmen2016}.
%This is especially problematic if the inter-event times are of interest \cite{Willekens2009}.
%Second, typically multiple updates need to happen at the same time step, e.g., the updates of multiple agents.
%The modeler must decide for an update scheme that processes these events in some order, and the choice of update scheme may have significant influence on the model's behavior \cite{Ozmen2016}.

%These issues can be avoided by employing \emph{discrete event simulation}.
%Thereby, events (in an agent-based simulation the actions of agents) are scheduled in continuous time, and time is not advanced in fixed-size steps, but always to the next event \cite{Law2014}.
%Specifically, we implemented the model using the Modeling Language for Linked Lives (ML3) \cite{Reinhardt2021}.
%ML3 was originally designed for agent-based demographic models, where the live-courses of interacting individuals are simulated.
%However, it is not limited to this application area.


%MODEL REQUIREMENTS

%To model credit demand the output should reveal a business cycle in accordance to relative volatility of GDP, investment and consumption \cite{Stock.1999,Napoletano.2006} and persistent fluctuations \cite{Burns.1946}.






EXAMPLES for model features:
\begin{comment}
Price = information for consumption
price = set via demand and competition. Whereas competition has assumed frictions, like bounded rationality and incomplete information about the best price. 


\begin{itemize}
    \item[1.] Agent/s involved: Firms
    \item[2.] Frequency: Continuous
    \item[3.] Rule based
    \item[4.] ML3 location: Line 247 to 360
\end{itemize}

\begin{figure}[h]
\begin{lstlisting}[language=ml3]
Agent/s involved: Firms
Frequency: Continuous
Waiting time expression: adaptive rate
ML3 location: Line 247 - 360
\end{lstlisting}
\caption{ML3-Features for supply mechanism}
\label{fig:}
\end{figure}
\end{comment}







%This paper introduces a methodological amendment for macroeconomic agent-based models (MABMs) in a new simulation environment with the purpose to analyze alternative monetary system regimes. The intention indicates three sub-aspects:\newline

Research gap:
ML3 is able to combine interbank network modeling (which is very granular = see Liu 2020) with macroeconomic variables

All other papers are step wise and discrete
-> Interbank markets do not work step wise. Reserves have to be cleared on a daily basis. Crisis or market anomalies can occur in a very short time frame (see shock in US money market or financial crisis)

FLAME is able to simulate on a simultaneous basis, but is still step wise and discrete.

Compare interaction profile of other MABM families when listing advantages of MABM in ML3 (cite Dawid)

Chicago plan = not sovereign money (still two circuit etc. See Huber)
Our model is mixture between various models seen in Dawid = mainly Gualdi (based on Delli Gatti) and Caiani = see Provenance!
Concurrent processes = measuring stability/resilience depends on network effects = occur via parallel concurrent processes! 
Galati 2012:
the resilience of the financial system depends in a non-linear fashion on its network
connectivity: while the likelihood of contagion may be reduced by greater connectivity, the potential
impact of a shock has a much larger scale (Gai and Kapadia, 2010; Nier et al., 2008).

potential expected benefit, because it provides higher quality to mime realistic dynamic due to higher interdependency level between economic mechanism. However, we cannot clarify the quality of macroeconomic policy experiments in comparison to a step-wise approach but see high potential in even more realistic analysis within the money market and its feature of imbalances that might arise from the co-evolution of interbank and credit markets and mutually reinforcing dynamic.  






%Research question
%Lin: this is not a research question, that something can be defined as something ... what is the problem you want to solve?
%First, in general a monetary system can be defined as the money issuance process of institutional interaction within an economy or network of economies. As already stated in Benes and Kumhof (2012), the analysis of the monetary system comes along with debates on the nature of money and who should control money issuance or how should it be organized.\footnote{For further details on the nature of money please see Benes and Kumhof (2012)...ADD further literature.} The analysis of alternative monetary systems shed new light on institutional and regulatory interplay of the current system with regard to systemic stability concerns. There are two contrary monetary systems that both claim to lead to a more stable financial system when implemented: Sovereign money and Freebanking system. 
%Shortly explain monetary systems and why it matters
%A sovereign money system (SMS) is also known as positive money and describes a money system under full money issuance control by the sovereign.\footnote{For further details see Huber, Jackson and Dyson and collaborators.} In contrast, a Free banking system (FBS) indicates a pure private money issuance regime and little or no sovereign interference.\footnote{For further details see...} \footnote{For a more detailed comparison see section\ref{discussion}.} 
%Lin
%Both systems come along with institutional changes which might be interesting to analyze for efficiency and effectiveness aspects of macroprudential policy within the current money system: A SMS can be defined as a two-tier single-circuit money system\footnote{Single-circuit means that there are no reserves circulating and only central bank money} and a FBS as a one-tier single-circuit money system.\footnote{One-tier means that there is no Central Bank involved and single-circuit means that only banking money is circulating.} Money issuance in the current system is mainly driven by credit creation via private financial institutions (see Bank of England (2014) and Bundesbank (2017))in a two-tier split-circuit system\footnote{Two-tier means a two-tier banking structure, consistent of central bank and banking sector. Split-circuit means the split of banking money in the public circuit and central bank money in the interbank circuit. For further details see Huber (2017).}\newline


%Third, 
In comparing alternative monetary regimes, it needs to be taken into account, that 
the stability conditions mentioned above, are related to the behavior of the respective monetary system to endogenous and exogenous shocks. Measuring stability conditions with regard to institutional system changes can be seen in Krug 2018, Van der Hoog (2018) and Popoyan 2019, who use various ways to analyze effects on the business or financial cycle. A more detailed discussion on stability measures is discussed in section\ref{discussion}.\newline


\begin{comment}
It can be concluded that related literature have no adequate implementation of a two-tier split-circuit system that reflects the current monetary system and serves as a benchmark for comparing various monetary regimes. The conclusion is drawn on the fact that relevant related MABM do not implement endogenous money theory according to the status quo\cite{BankofEngland.2014,Bundesbank.2017} which is fundamentally crucial to analyze monetary systems. For example, the analysis of the reserve requirement level, leads to different interpretation when assuming a strong effect of the money multiplier. Other MABM miss the focus of the financial cycle or do not implement an adequate interbank market to address liquidity risk.

What is missing in model with regard to monetary system?
Popoyan
= no investment cycle that reflects inflation and crisis cause (bubble creation). Which is crucial to investigate stability level of alternative monetary systems. 

= no full reflection of endogenous money/money issuance. LCR set the restriction to bank money supply, but has little impact on the monetary base according to 
Howitt (2012) is not correct = no conflict between monetary base fluctuations and money supply, because money supply originates by endogenous credit supply and the base money is adapting accordingly. The nominal anchor (main refinancing operation rate) dictates indirectly the money supply. LCR is not dictating macroeconomic behavior, only in crisis. But per se it stabilizes the liquidity management of banks.
= bonds are not credit created?

accessibility? Model insights and behavior/validation are not transparent


Van der Hoog
no endogenous money
money multiplier = we do not assume according to BoE and Bundesbank.
no interbank market = no differentiation between banking money and central bank money

Krug
small population
no investment mechanism! But this is crucial to replicate pro-cyclical credit cascades.
no bubble creation (minsky moment), credit cascades

Caiani/Schasfoort
missing macroprudential policy restrictions or general credit creation potential

Reissl?
no overnight interbank market  = too simplified and no effect on model

Growth defining by firm capacity growth is not per se needed to investigate stability level of alternative monetary systems and comes along with higher model complexity. For simplicity the production capacity is always limited in the basis model at hand. The focus is set on credit cascades and pro-cyclical behavior of firm investments. 
\end{comment}


\begin{comment}
\begin{itemize}
    \item Business cycle and financial cycle
    \item Systemic risk features (time-varying and cross-sectional risk) Mime inherent financial (in)stability = see Stallinga
    \item Features of financial stability (stability and efficiency measures)
    Fractional reserve system
    \item Fiat and endogenous money creation according to prevailing opinion \cite{BankofEngland.2014,DeutscheBundesbank.2017}
    \item Money multiplier
    \item Payment system or differentiation between basis and banking money (two-tier split-circuit system (see citation in finland)) which shoud include monetary policy institution and related interbank market (liquidity constraints, knock-on effects, bun runs)
    \item External credit creation limitation: macroprudential regulatory framework
    \item Fundamental monetary transmission process (including financial accelerator)
    \item Bundesbankkritik zu Vollgeld
\end{itemize}
\end{comment}


Related literature


%fill matrix and describe
%Caiani = 3. p.a. because bank liquidity risk (interbank market) is no basic liquidity management scheme; 4.1. p.a. no integrated overnight payment system according to mime liquidity constraints TARGET2 or at least open market transactions within a monthly period. There is no indication that the Central Bank adjust the interbank bank rate via reserve restriction. 5. p.a. because no minimum capital requirement, only counter-cyclical capital buffer is applicable, 7. p.a. code is accessible but not a DSL

%van der Hoog = 3. p.a. because liquidity management of banks, 4.1. p.a. no interbank market, 4.2. p.a. endogenous money supply is not in line with Bank of England. = reserve requirement is not a credit restriction (money multiplier), 7. p.a. no DSL

%Krug = 2. p.a. because of no distinct investment mechanism 

%Popyan = 2. p.a. no distinct investment mechanism, 4.1. p.a. no distinct differentiation between money and credit. Furthermore, it is not clear how the Central Bank organize open market operations to influence interbank rate.

%Alexandre and Lima? = not included, because no interbank market.

%accessibility = key issue is that central bank behavior has to be modelled in various ways in combination with various other mechanism alternatives that can be easily implemented and replicated by readers.
%=other models are accessible as well, but not to the desired degree. This model uses a simulation framework that makes replication more simple


The CATS family (Complex Adaptive Trivial Systems) sets up a descent basis for fully-fledged agent-based models and serves as a benchmark and inspiration for various MABMs. Assenza et al.\cite{Assenza.2018} present a split-circuit financial system and conclude that considering interbank extensions in MABM affects the dynamics of macroeconomic model behavior. In comparison to the baseline scenario the Taylor rule is most effective in stabilizing macroeconomic output (GDP and related volatility and crises circumstances) in relation to the tested macroprudential policies.

The models of Caiani et al./Schasfoort et al., van der Hoog (ib.), Krug (ib.) and Alexandre and Lima (ib.) are interpreted as stock-flow consistent due to Godley and Lavoie\cite{Godley.2007} (see also Caverzasi and Godin\cite{Caverzasi.2015}) and Nikoforos and Zezza\cite{Nikiforos.2017}. The Stock Flow Consistent approach takes fund flows between financial and real sector into account and integrates responses and interrelations of balance sheet information from economic agents.



This paper serves as a methodological amendment to macroeconomic agent-based models (MABMs) with the purpose to analyze alternative monetary system regimes and related institutional changes within the current financial system of advanced economies and the implication of rebound effects with regard to systemic stability. 
%Lin: this is a bit late to discuss this typically  is done at the beginning
%To specify the purpose of this paper the objects under investigation have to be further disambiguated and discussed.


%Details des Modells - konkret auf das Modell beziehen. Was bringt mir das Modell? Im Vergleich zu anderenden Modellen. Auf das Ergebnis gemünzt. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Alternative monetary system regimes}\label{monetarySystem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Lin: I am not sure how this relates to the findings, assumptions or your modeling efforts ... this appears far too general and little related to the paper at least from my point of view. this is more or less what you already stated ... 
A monetary system can be defined as the money issuance process of institutional interaction within an economy or network of economies. As already stated by Benes and Kumhof\cite{Kumhof.2012}, the analysis of the monetary system comes along with debates on the nature of money and who should control money issuance or how should it be organized. The analysis of alternative money issuance regimes shed new light on institutional and regulatory interplay of the current system with regard to systemic stability concerns. There are two contrary monetary systems that both claim to lead to a more resilient financial system: Sovereign money and Free banking system.

The Sovereign money system is also known as positive money and describes a money system under full money issuance control by the sovereign. Proponents of sovereign money criticize the private credit creation dominance which is indicated as a main driver for toxic exuberant pro-cyclicality, leading to unintended and preventable severe boom and bust cycles. Sovereign money, inter alia, should serve as a limit/buffer for boom and bust periods. Bank liquidity crisis would become highly improbable due to full-fledged Central Bank money which conduce to an inherently insolvency protection for bank runs. The Central Bank has direct control of money supply which should yield in more effective anti-cyclical monetary policy enforcement and lower limits for asset price bubbles. Further details are elaborated by Huber\cite{Huber.2017}, Jackson and Dyson\cite{Jackson.2015} and collaborators.
%TODO: conflation of credit and money is a dysfunctional feature and the market power to  influence the aggregate money supply proactively. Assumption that inflation targeting with interest rate policy is not effective. Transmission to money supply politic. Assumption that central bank has all relevant information and orientation to output potential and that private market power distort a optimal money supply politics, which can be rectified by a sovereign system. 

%Lin: how can the different banking systems be implemented in ML3 or are they already I do not see this here 
In contrast, a Free banking system indicates a pure private money issuance regime with little or no sovereign interference. Proponents of Free banking are supportive for a full market based monetary system that is inherently stable due to the absence of statutory distractions. It is criticized that Central Banks do not know \qq{optimal} money supply due to lagged macroeconomic behavior and data availability which in turn distorts market interest rates through non-optimal monetary policy. Free banking reduces misallocations and asset price bubbles via automatic market stabilizers\cite{Paniagua.2016}. In principle the research idea is a theoretical reincarnation of the debate between banking and currency school in the 19th century with the evolutionary difference of today's fiat money regime instead of a gold standard.

The current money issuance regime is a two-tier split-circuit system which could be described as a mixture between a sovereign money and Free banking regime. A two-tier banking structure is consistent of Central Bank and private banking sector. Split-circuit describes the dichotomy of banking money in the public circuit and central bank money in the interbank circuit\cite{Huber.2017}. A sovereign monetary system can be defined as a two-tier single-circuit money system and Free banking as a one-tier single-circuit money system. A single-circuit flow incorporates only one single money type (either circulating central bank money or bank money). One-tier is classified here when no Central Bank is involved. 

%Lin: the above needs to be substantially reduced, sharpened and the relation to your model needs to be clarified

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System stability}\label{stability}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As stated in the previous paragraph alternative monetary regimes proclaim a more stable macro-financial system. There is no standardized definition of financial stability, but can be generally captured as the absence of dysfunctional behavior within the financial sector\cite{Gadanecz.2009,Schinasi.2004} or \qq{[...] its ability to
perform its key functions remains well within a set of tolerable boundaries — defined over a set of measurable variables [...]} \cite{Schinasi.2004} which are defined below.

%Lin the following appears to be redundant, please reduce. 
%As described in the introduction MABMs are predestined to analyze instability macroeconomic system features that emerge endogenously. In addition, adverse external shocks might occur that have to be processed and absorbed by the macroeconomic system (shock-absorptive capacity). Hence, alternative monetary regimes within a MABM implementation have to be analyzed according to endogenous and exogenous driven shocks in relation to the facilitative and efficiency-enhancing role of the financial system\cite{Schinasi.2004}.

To measure (in)stability conditions, the corresponding MABM has to incorporate the origination of systemic risk. According to Borio\cite{Borio.2003}, Bank of England\cite{BoE.2011} and Galati and Moessner\cite{Galati.2012} systemic risk is classified in time-varying and cross-sectional risk. Time-varying risk belongs to pro-cyclical behavior of the financial sector, caused by solvency, liquidity and contagion risk \cite{Krug.2015} and feeding the financial cycle \cite{Borio.2012a}. Cross-sectional risk is related to the structural composition of the financial sector, such as distribution of risk within the financial network, co-varying risks across balance sheets, systemically important financial institutions and opacity of complex network interdependencies \cite{Krug.2015}.
%Lin: as derived is odd english also it is not performance but simulation results and again the relation needs to be strengthened how does the different types of risk relate (so what you describe above) to what you have done, could all three types of risk be integrated, this needs to be discussed in more detail. 
%As derived from the model description and performance (Section \ref{model}) and \ref{output} respectively), 
The present model can mime systemic risk causes which are addressed by money issuance regime proponents in relation with macroprudential policy (see Section \ref{output}).
%TODO: no fristentransformation = Vorteile that should lead to more stable boom-bust cycles, increased private savings and low interest level on capital markets that and lead to steeper growth path. Disadvantages = no Fristentransformation could lead to welfare deficits. Long term oriented investors and short term oriented depositors are by far less matchable. = efficiency loss. 

%Lin: you write sometimes very complicated sentences ...
%This model follows the conclusion of 
As suggested by Borio\cite{Borio.2012a}, 
the financial cycle is modelled in the way that \qq{[...] the financial system does not just allocate, but also generates, purchasing power, and has very much a life of its own [...]}, which is in line with the non-neutrality assumption\cite{Rochon.2003} in order to analyze effects of alternative monetary regimes on systems' stability. 
%Lin: how does your the financial system in your model generate purchasing power, please be more concrete. 
The financial cycle in this MABM has a strong focus on the credit cycle, which is in line with Aikman\cite{Aikman.2015}, Dell'Ariccia\cite{DellAriccia.2012}, Jorda\cite{Jorda.2011} and Schularick\cite{Schularick.2012} and is highly demand driven to show direct influence of money issuance. 
%Lin: has the credit cycle been described formally? 
In combination with the assumed model restriction (see Section \ref{assumptions})
%Lin: which of the assumptions in particular, please make it a bit more concrete
this model serves as a basis for the analysis of money issuance regimes and its effect on the credit/financial cycle. As a consequence, the business cycle and financial cycle are synchronized (see table \ref{tab:SF5}) which reduces another interfering layer for analysis of alternative monetary system. Financial fragility is also driven by network effects of the credit and interbank market\cite{Iori.2018}, which can be taken into account via ML3. 
The basis model assumes homogeneous network structure of banks and firms, which tend to be more favorable for the stability of the system\cite{Iori.2006,Battiston.2012,Lux.2016}.
%Lin: this should be done at the end, but the sentence structures are overly complicated, sometimes it is not clear what is meant (rather vague statements), and redundancies exist, e.g., the sentence below, the first part I do not understand and the second part needs an example how is it possible for the model to reflect this ... 
%please use at the end (if the structure is OK, and everything is as it should be some program to polish the English). 
Furthermore, the impact of the firm-bank network on systemic risk, e.g., % to reflect ?????
the contagion between financial sector and real economy\cite{Lux.2016}, can be reflected by the model. 

System stability measures within MABM are used for example in Popoyan\cite{Popoyan.2019}, Krug\cite{Krug.2018} or van der Hoog\cite{vanderHoog.2018}. Common measures are output gap, unemployment, inflation, bank fail frequencies, leverage ratio (credit-to-GDP ratio and/or debt-to-equity ratio of banks), severity of recessions and cumulative loss of output during recessions. To test the systems reaction to external shocks, Ramey\cite{Ramey.2016} gives a pre-defined overview for monetary, fiscal and technological shocks in DSGE models.



To Criteria 2
When indicating the influence of monetary regime changes the model behavior should 
influence of money issuance and long term restriction

=credit size is pre-defined and closely related to production capacity = no rally and speculative credit bubble = firms try to exploit profits
= explicitly fueling credit bubbles, credits overshoot productive utilization of capital. A normal credit supply would mean, that all invested capital would flow into production/productive sphere. However, firms face uncertainty regarding optimal equilibrium of supply and demand. = gap between real and nominal values.

Huber: As the banking and financial industries have a strong incentive to extend
their business as much as possible and as the central banks have stopped asserting
control over bankmoney, the ensuing dynamics of banking and fi nancial
markets tend to cross critical lines, thus overshooting. Th is results in infl ation
(in recent years primarily in newly industrializing countries) and more markedly
in asset infl ation, bubble building, fi nancial over-investment and overindebtedness,
discharging in crises that aff ect everyone.

Thus, the final restriction on monetary and financial expansion is set by the gravitational force of real economic productivity. Real productivity, actual output and income, determines the economy’s carrying capacity for financial assets and debt. = gap between real and nominal values.

+ over borrowing due to production potential - credits serve also for speculative reasons. 

whereas in Mak(h)ro loan size can overshoot production capacity because investments are also used in a speculative way in the sense that firms enter into a rally to gain higher profits while not knowing how much investments can be processed in a productive way. This leads to a model behavior with very strong pro-cyclical amplitudes. = can be seen in higher volatility of investments which are mainly financed by credits in Figure 5 \ref{fig:SF1} and Krug \cite{Krug.2018}.
However, model behavior cannot be precisely compared, since the MABM of Krug and Popoyan are not accessible or replicable. 

+ OUR MODEL constantly produces severe recessions caused by credit bubbles. This makes the identification of systemic risk features more straight forward. 

In boom phases there are more investments that can be transferred into general demand and in bust phases less investments are created than necessary to keep the economy stable.

The other related MABMs in Table \ref{tab:literatureMatrix} do not implement speculative or unproductive credits and let firms go bankrupt when debt obligations cannot be met and outstanding loans are higher than financial wealth. Hence, unproductive credits do not play a role or only partially and credit cycle may not be observed in the same severity like discussed above. 



Credit demand is generated via constant adaption to demand impulses by households. 
Our contribution is the implementation of an investment behavior that generates firm investment profits depending on aggregate firm investment behavior and/or good/asset prices. This mechanism do not need capital firms to generate investment demand and has the effect of overshooting credit demand/supply as stated by Huber \cite{Huber.2017}. 



%Whereas the business cycle 

%The difference of Mak(h)ro to other MABM is a separate specification between consumption and investment behavior without using capital firms unlike related MABM $a$ and $b$. 

We consider a financially fragile economy with a high degree of financialization
in which (non-financial) firms need loans from commercial banks to service their
various financial commitments: to produce a final consumption good, to service their
outstanding debt, and to make long-term investments. Along the business cycle the
economy follows the dynamics of the Minsky base cycle in which firms traverse the
various stages of financial fragility, i.e. hedge, speculative and Ponzi finance

%The business cycle according to Stock and Watson \cite{Stock.1999} can be replicated by all related MABM.  
model feature to mime overshooting money supply. = define overshooting
Overshooting = over borrowing or debt overhang
financial fragility and macroeconomic outcome
monetary system as one crucial aspect of financial fragility (proponents of alternative monetary systems)
A recurring theme in all these empirical studies seems to be that higher financial
leverage raises the vulnerability of an economy to shocks, and leverage functions as a
propagation mechanism for other destabilizing effects such as the financial accelerator
(Bernanke and Gertler 1990). If left unattended, such vulnerable economies may enter
into a balance sheet recession (Koo 2009) with the ensuing damaging effects of a
debt deflation (Fisher 1933). Or, possibly even worse, it may result in long periods of
secular stagnation (Summers 2014).
8

Business cycle with alternative investment cycle same, credit cycle the same behavior but bubble emergence is different. Here investment is price sensitive. Investment profits are only generated via price increases which arise from demand = here allows overshooting and zombie lending. How to define overshooting? = price mechanism?
investment when expected profit is positive = when prices rise, prices do not follow a wage-price spiral, but a asset price behavior since wages are fixed. Means, prices and investments rise even when production capacity is fulfilled. Has an effect like asset price bubbles = zombie lending = overshooting (also via financial accelerator = price increases work as profit expectation booster, higher profits = higher equity and liquidity = higher collateral and higher creditworthiness, also via history of profits = expectation of profits)
Here...credit demand mechanism is different = 

There...in Krug and Popoyan = wage is demand and price driver which is indirectly fed via expecting production capacity
= no zombie lending = firms exit when debt obligations are not met. Same in Popoyan and Caiani. 

= demand via household demand. Higher wages = higher demand. 
= here, investment demand drives price bubble = distinct overshooting behavior
= overshooting via net present value = expecting profit which increase via higher demand. In boom phases here causal effect is that demand constantly overshoots aggregate production capacity = price increase. Hence investments generate positive yield and further investments are initiated. Investment rally is triggered. 
Debt overhang?


In Caiani = 
investment demand via production capacity - impact via demand and expected production capacity needed. Exact difference = no distinct zombie lending and asset price bubble behavior/phenomenon.  


%The first contribution of the presented model to the MABM literature is set out in criteria 2 in Table \ref{tab:literatureMatrix}, which requires the implementation of a model feature to identify overshooting credit behavior of banks as stated in Huber \cite{Huber.2017}. The difference lies in the investment behavior of firms which mainly define credit supply. For example, Caiani et al. and Schasfoort et al.



%Caiani/Schasfoort:
%Not designed to mime credit overshooting or credit bubbles as stated in Huber \cite{Huber.2017}, when firms 
%redit creation potential in combination with capital requirements
%In this model, firms seek investment opportunity = dependent on other behavior





















Especially the MABM of Krug \cite{Krug.2018} mime the current monetary system in great detail. A more detailed comparison  Are described in the following 

%Lin: I do not understand all full fledged mas would be long to this ... what makes up a CATS, please as below you write about another family that does not belong to this --- also do you only recite here findings of the 2018 paper, if so you need to clarify this ... 
The model can be categorized to the CATS (Complex Adaptive Trivial Systems) family \cite{Dawid.2018} which sets up a descent basis for fully-fledged agent-based models and serves as a benchmark and inspiration for various MABMs. For example, the work of Gualdi et al. \cite{Gualdi.2015} is related to CATS which in turn is partly a basis for this model (Section \ref{supply}, \ref{labor} and \ref{consumption}).
Table \ref{tab:literatureMatrix} summarizes the match of related model mechanisms to the desired criteria described in Section \ref{criteria}. Our model is partially build on the %sound 
work of Caiani et al. \cite{Caiani.2016} and Schasfoort et al. \cite{Schasfoort.2017} (Section \ref{creditMarket}) and is enlarged by a full-fledged payment scheme according to the ECB framework (Section \ref{interbank}) which includes a basic bank liquidity management with open market transactions to identify bank liquidity constraints (criteria 3. and 4.1). Furthermore, our research purpose requires the incorporation of capital requirements which are only partly implemented by Caiani et al./Schasfoort et al. \cite{Caiani.2016,Schasfoort.2017}. %documentation: https://github.com/S120/jmab

%Popoyan and Krug = no distinct opportunity to mime asset price inflation via investments. Important because proponents of sovereign money claim that the reduction of private money issuance possibility leads to lower asset price inflation. = overshooting money supply that cause price bubbles. 



%Lin: clarify what is the relation to our model? 
The second relevant MABM family is a branch from the EURACE project \cite{Dawid.2018}, known as Eurace@Unibi (EUBI). The EURACE project is based on a \qq{flexible large-scale agent modeling environment} (FLAME) with the aim to reconstruct the European economy within an agent-based model \cite{Deissenberg.2008}. Van der Hoog \cite{vanderHoog.2018} presents a sound and comprehensive model to shed light on the relation between different credit market- and banking regulations and macroeconomic performance. However, the author does not differentiate between money and credit within a two-tier-circuit system \cite{BankofEngland.2014} which is a fundamental feature to identify interdependencies between money issuance and macro-financial stability (criteria 4.1 and 4.2). This circumstance also influences systemic risk that evolves from maturity transformation management (criteria 3).
%van der Hoog = 3. p.a. because liquidity management of banks, 4.1. p.a. no interbank market, 4.2. p.a. endogenous money supply is not in line with Bank of England. = reserve requirement is not a credit restriction (money multiplier), 7. p.a. no DSL
%Lin: in addition to what?
In addition, van der Hoog\cite{vanderHoog.2018} uses the model to implement a full reserve banking scheme according to Douglas et al.\cite{Douglas.1939}, which can be classified in the same family as a sovereign monetary system. 
%Lin: is the following of importance for the story line and what relation does this have to your modeling efforts?
%However, the definition and the corresponding features of the \qq{Chicago Plan for Monetary Reform} to be claimed as sovereign money is misleading. The \qq{Chicago Plan for Monetary Reform} is not sovereign money, since sovereign money implicates a single circuit flow and has not the strict ingredient of full equity finance to Cochrane\cite{Cochrane.2014}. A full equity finance restriction completely diminishes the money issuance mechanism within the financial system and is not compatible with the endogenous money assumption according to Bank of England\cite{McLeay.2014} and Bundesbank\cite{DeutscheBundesbank.2017}. 

%maturity transformation concerns are not addressed that could hamper welfare via efficiency losses
%identification of stability conditions in comparison to current system. For example, liquidity constraints, pro-cyclical asset evaluation and possible runs on refinancing assets and corresponding capital requirements
%only equity funding, debt financing is disregarded.
%Role of monetary policy is not modeled in accordance to a strict money supply policy 
%The third
An even more detailed two-circuit monetary framework in MABM is presented in Krug\cite{Krug.2018}, which is based on the UK Sterling Monetary Framework of the Bank of England in order to analyze the impact of the interplay between macroprudential schemes and monetary policy on financial stability. As in van der Hoog\cite{vanderHoog.2018} it is concluded that preventing extensive credit growth leads to less severe financial imbalances and a more stable macro-financial behavior.
%Lin: and how does relate to our model?

%Krug = beside the financial sector our model uses alternative real sector mechanisms with an accentuate on the investment cycle. The investment cycle is separated from household consumption which allows a non-concurrent demand structure that influences the business cycle performance and in the consequence the financial stability condition.

The fourth relevant MABM family is the medium-sized MABM developed by\cite{Ashraf.2011} and is extended by Popoyan et al.\cite{Popoyan.2017,Popoyan.2019} and investigates the interaction between Basel II and III macroprudential frameworks and different types of Taylor rules in order to analyze financial instability. The model simulates a basic real business cycle without an investment cycle. The financial market sub model includes a comprehensive fractional reserve system and is able to give hints for different financial market regulations schemes and the impact on financial stability.

%Popoyan = 2. p.a. no distinct investment mechanism, 4.1. p.a. no distinct differentiation between money and credit. Furthermore, it is not clear how the Central Bank organize open market operations to influence interbank rate.

%Lin: what does it mean that a similar result can be interpreted? and is this interesting in comparison to what our model is?
%A similar result can be interpreted in\cite{Alexandre.2017} who conduct a similar research setting. The authors state that macroprudential policy, like Basel II, is highly effective in dampening financial imbalances by the negative relationship of non-performing-loans to credit ratio and output and price volatility.
%Alexandre and Lima? = not included, because no interbank market.

%Lin: the listing of relevant MABMs is without a discussion how this relates to our model not very helpful, particularly related work at the end of a paper gives the opportunity to clearly describe what one has done in comparison to already existing work, this is not the case here. 
Further relevant MABMs that follow a Stock-Flow Consistent integration are developed by Reissl\cite{Reissl.2020} and Schasfoort\cite{Schasfort.2017}.

Reissl\cite{Reissl.2020} presents a hybrid agent-based stock-flow-consistent model. Hybrid agent-based models combines aggregated modeled sectors with micro-funded agent-based sectors. For further research see Assenza et al. \cite{Assenza.2007,Assenza.2013,Assenza.2019}, Michell\cite{Michell.2014}, Pedrosa and Lang \cite{Pedrosa.2018} and Botta\cite{Botta.2019}. The reason for aggregating certain sectors within an agent-based model is based on the idea to circumvent complexity of a multi-agent model with its pitfall of non-identifiable impact mechanisms between various behavior of agents and their variables and parameters\cite{Assenza.2013}. Results are in line with those stated above. An adequate combination of monetary and prudential policy lead to less macroeconomic fluctuations in the model.

%Lin the following is redundant. also it reads as if you only recite what David et al. already did more extensively, the related work Section needs to be revised to discuss it from the point of view of comparing your model to those already existing ones. what can your model do that others could not or what did you do differently ----  
%Related literature is mainly related to models that implemented interbank and credit markets to represent the monetary system. More related literature with regard to monetary policy can be found in Dawid and Delli Gatti\cite{Dawid.2018}.


Krug = constant overinvestment with buffer function. Prices are strictly bound to wage dynamic. Hence, no price bubbles and related credit bubble can be identified to the desired transparent mechanism (\textif{requirement 2} in Section \ref{requirements}).




source of credit demand = wage driven and wage-price spiral = no (asset/investment) price cascade which drives overshooting credit cycle (demand and supply) = no price and credit bubbles and identification of productive and unproductive credits to prevent a rally for extend production capacity.

Krug = focus on influence of central bank on inflation.
Here, focus on influence of money supply on (overshooting) credit supply. Which might lead to similar output (when comparing validation), but to different identification of credit cycle behavior which is more transparent in Mak(h)ro ABM. However, the presented basic model misses a wage dynamic in accordance to make the main causes of overshooting credit behavior transparent and identifiable. Via ML3 this can be expanded in a transparent way. 

no collateral and extrapolation of expected debt obligation = no financial accelerator

Credit growth related to increasing production unit costs via higher wage expenses which in turn generates demand and are constantly rising via labor productivity and expected inflation. which in turn influences target production and = influence of money is not as clearly identifiable as an investment approach followed by Mak(h)ro.

Here, credit growth or specifically its pace is identifiable by price increases and available credit supply potential by banks in relation to creditworthiness of firms.  

Krug, Popoyan = focus on relation between monetary policy and financial stability.
Here focus on monetary system and its impact 

Furthermore, speculative borrowing like van der Hoog.

overshooting? = bank behavior to expand or exploit?
= important to model possible behavior rule for Central Bank to control money supply in sovereign monetary system.



Popoyan = no clear identification of credit supply to financial fragility. 




%identification of credit potential and unproductive credits, speculative investments which are not absorbed by production capacity. 

%However, the financial cycle (requirement 2) or credit cycle, which is highly intertwined with the business cycle, reveals a model behavior differences that partly arise from the implementation of productive and unproductive credit supply (see Section \ref{requirements}). The separate investment mechanism (Section \ref{investment}) amplifies the pro-cyclical credit cycle effect and mimes a crisis dynamic in accordance to Minsky \cite{Minsky.1978, Minsky.1982}. This behavior can be observed within the MABM of van der Hoog \cite{vanderHoog.2018} and the present model \qq{Mak(h)ro}. 

ENTSCHEIDEND: Caiani and van der Hoog = could 
influence of monetary system on (overshooting) credit supply, which can be mimed by Caiani and van der Hoog. However, Caiani does not incorporate 

%Other related MABM in Table \ref{tab:literatureMatrix} show either smooth financial cycles \cite{Caiani.2016,Schasfoort.2017,Popoyan.2019} or only few severe credit bubbles \cite{Krug.2018}. Unproductive credit production does not play a role or only partially. Our model mainly generates credit bubbles that come along with severe GDP downturns which makes the identification of systemic risk features more transparent.
%identification is important to measure effect of productive credits (asymmetric information) under aspect of comparing a monetary regime shift.
%sovereign money/free banking = since it is not clear if this system can prevent unproductive credits and credit bubbles in a significant way.

%TODO: Krug can replicate crisis dynamic, but it is not clear why credit cycles become more severe over time.

